On Bonus-Based Exploration Methods in the Arcade Learning Environment

Research on exploration in reinforcement learning, as applied to Atari 2600 game-playing, has emphasized tackling difficult exploration problems such as Montezuma's Revenge (Bellemare et al., 2016). Recently, bonus-based exploration methods, which explore by augmenting the environment reward, have reached above-human average performance on such domains. In this paper we reassess popular bonus-based exploration methods within a common evaluation framework. We combine Rainbow (Hessel et al., 2018) with different exploration bonuses and evaluate its performance on Montezuma's Revenge, Bellemare et al.'s set of hard of exploration games with sparse rewards, and the whole Atari 2600 suite. We find that while exploration bonuses lead to higher score on Montezuma's Revenge they do not provide meaningful gains over the simpler $\epsilon$-greedy scheme. In fact, we find that methods that perform best on that game often underperform $\epsilon$-greedy on easy exploration Atari 2600 games. We find that our conclusions remain valid even when hyperparameters are tuned for these easy-exploration games. Finally, we find that none of the methods surveyed benefit from additional training samples (1 billion frames, versus Rainbow's 200 million) on Bellemare et al.'s hard exploration games. Our results suggest that recent gains in Montezuma's Revenge may be better attributed to architecture change, rather than better exploration schemes; and that the real pace of progress in exploration research for Atari 2600 games may have been obfuscated by good results on a single domain.

==> evaluation_protocol.tex <==
\section{Evaluation protocol}
We evaluate previously introduced exploration methods along two main axes, the first one being sample efficiency i.e. how quickly can they get to closer to the optimal for a particular environment.
While it is a key objective for exploration methods, published agents are often trained under different regimes making it hard to an apples to apples comparison.
They often employ different reinforcement learning algorithms, varying quantity of training frames or inconsistent hyperparameter tuning.
As a remedy, we fixed our training protocol and trained bonus-based methods with a common agent, the Rainbow implementation provided by the Dopamine framework \citep{castro2018dopamine} which includes Rainbow's three most important component: $n$-step updates \citep{mnih2016asynchronous}, prioritized experience replay \citep{schaul2015prioritized} and distributional reinforcement
learning \citep{bellemare2017distributional}.


The second axis is generality, the initial goal of the ALE was to promote the design agents with a general competency in a variety of different domains.
% Only few games were to be used for training set and the remaining ones would be used for evaluation.
% Nonetheless, it has become common to tune hyperparameters on \textsc{Montezuma's Revenge} only, then evaluate on the ALE games classified as \textit{hard exploration games with sparse rewards} in \citeauthor{bellemare2016unifying}'s taxonomy: 
% \begin{itemize}
%     \item[--] \textsc{Freeway}, \textsc{Gravitar}, \textsc{Solaris}, \textsc{Venture}, \textsc{Private Eye}.
% \end{itemize}
% While this may be due to limited computational resources doing so however may come to a price on easier exploration problems as we will see later on.
% For this reason we chose to also evaluate performance on the original Atari training set\footnote{\textsc{Freeway}, \textsc{Asterix}, \textsc{Beam Rider}, \textsc{Seaquest}, \textsc{Space Invaders}} as well as the remaining Atari games. 
The current practice followed by the community has been to tune agents in \montezuma{}. We evaluate if \montezuma{} is indeed predictive of performance in other settings. Moreover we evaluate how well these algorithms across all Atari games to understand the impact these bonuses have in other domains
